Low-rank finetuning for LLMs: A fairness perspective

Low-rank approximation techniques have become the de facto standard for fine-tuning Large Language Models (LLMs) due to their reduced computational and memory requirements. This paper investigates the effectiveness of these methods in capturing the shift of fine-tuning datasets from the initial pre-trained data distribution. Our findings reveal that there are cases in which low-rank fine-tuning falls short in learning such shifts. This, in turn, produces non-negligible side effects, especially when fine-tuning is adopted for toxicity mitigation in pre-trained models, or in scenarios where it is important to provide fair models. Through comprehensive empirical evidence on several models, datasets, and tasks, we show that low-rank fine-tuning inadvertently preserves undesirable biases and toxic behaviors. We also show that this extends to sequential decision-making tasks, emphasizing the need for careful evaluation to promote responsible LLMs development.

==> sections/results_classification.tex <==
%!TEX root=../main.tex

Next, we focus on the popular task of using language models for downstream purposes, particularly, the classification of text sequences. This task can be performed by serializing sequential data into natural language sentences \citep{HegselmannBLAJS2023AISTATS} or by adopting existing sequential natural language data. Influenced by research on the impact of a model's representational power on fairness \citep{DasRF2024ICML}, we aim to assess the implications of parameter-efficient fine-tuning methods on fairness in these sequential data tasks.

\begin{figure}[!t]
%\vskip 0.2in
\centering
  \includegraphics[width=0.99\textwidth]{figures/Fig4.pdf}
  % \begin{subfigure}[b]{0.325\textwidth}
  % \centering
  % \includegraphics[height=105pt]{figures/gpt2_imdb_all_ranks.pdf}
  % \caption{IMDb dataset}
  % \end{subfigure}
  % \begin{subfigure}[b]{0.65\textwidth}
  % \centering
  % \includegraphics[height=105pt]{figures/gpt2_sst2_all_ranks.pdf}
  % \caption{SST2 dataset}
  %\end{subfigure}
\caption{Disparate impact of fine-tuning with \gls*{lora} on sentence classification task for \textsl{IMDb} (left) and \textsl{SST2} (right) datasets, when the model penalizes some classes or groups more than others. The $y$-axis is group accuracy, while the $x$-axis is the size of the minority group as a proportion of the majority group at different levels of downsampling. 
The underlying pre-trained model is \textsl{GPT-2} fine-tuned for 5 epochs.}
\label{fig:lora_seq_gpt2}
\end{figure}

\paragraph{Potential disparate impacts in LoRA fine-tuning.}
We next provide evidence that LoRA methods may exacerbate the accuracy disparities between overrepresented and underrepresented groups. We explore this issue by analyzing accuracy parity and the harmful bias gap as defined in \Cref{sec:experimental_setup}. 

The analysis is visualized in \Cref{fig:lora_seq_gpt2}, which %compares the performance of LoRA fine-tuned models across different ranks and a regular fine-tuned model on both \textcolor{red}{majority} and \textcolor{teal}{minority} groups, defined relative to the labels (positive or negative statements) within the dataset. The x-axis represents the balance ratio, helping to assess fairness in the decision-making process.
compares the performance of LoRA fine-tuned models (dashed lines) across different ranks and a regular fine-tuned model (full lines) on both majority (\textcolor{red}{red colors}) and minority (\textcolor{teal}{blue colors}) groups 
within the considered dataset: \textsl{IMDb} (left) and \textsl{SST2} (right). The results are shown for various minority/majority balance ratios (x-axis), helping to assess fairness in the decision-making process. 
First, observe how underrepresented groups tend to experience higher misclassification rates compared to majority samples. Note also that the relative size of each group during the fine-tuning phase significantly affects the fairness outcomes of the final models, up to the point where the regular fine-tuned models are able to neutralize unfairness, in the balanced data cases. 
Second, and perhaps more importantly, notice how the rank of LoRA controls the disparity impact gaps between majority and minorities. In particular, lower fine-tuning ranks are associated to much higher accuracy gaps.

These disparities are further highlighted in Table \ref{tab:class_llm}, which details the harmful bias gap (HBG) for the minority group and the accuracy parity (AP) scores for models \textsl{OPT 1.3B} and \textsl{GPT-2} across the \textsl{IMDb} and \textsl{SST2} datasets. The table reveals a clear pattern where both unfairness metrics (where lower values are preferred) of the LoRA models gradually align with those of the regular fine-tuned model (RFT) as their fine-tuning ranks increase. 

\begin{table}[!htb]
  \centering
  \resizebox{\textwidth}{!}{
   \begin{tabular}{l l | r r r r r r r r}
    \toprule
            & & \multicolumn{2}{c}{\bf GPT-2 on IMDb} 
              & \multicolumn{2}{c}{\bf GPT-2 on SST2} 
              & \multicolumn{2}{c}{\bf OPT 1.3B on IMDb}
              & \multicolumn{2}{c}{\bf OPT 1.3B on SST}\\
    $\nicefrac{\textbf{Maj}}{\textbf{Min}}$ 
              & {\bf Rank} & {\sl HBG} $\downarrow$(\%) & {\sl AP} $\downarrow$(\%)
                     & {\sl HBG} $\downarrow$(\%) & {\sl AP} $\downarrow$(\%) 
                     & {\sl HBG} $\downarrow$(\%) & {\sl AP} $\downarrow$(\%)
                     & {\sl HBG} $\downarrow$(\%) & {\sl AP} $\downarrow$(\%) \\
    \midrule
                          & 2   & 3.4 & 14.5   & 1.8 & 17.4   & 1.9 & 7.2   & 0.3 & 6.9 \\
    \multirow{1}{*}{$\nicefrac{50}{50}$} 
                          & 8   & 2.0 & 13.4   & 0.5 & 19.5   & 0.2 & 5.9   & 0.7 & 7.7 \\   
                          & 64  & 0.8 & 10.3   & 0.9 & 14.2   & 0.1 & 6.5   & 0.7 & 7.7 \\
                          & RFT & $-$ & \bf{11.2}   & $-$ & \bf{ 8.8}   & $-$ & \bf{5.9}   & $-$ & \bf{7.4}  \\
                          \cline{1-10}\\[-0.8em] 
    
                          & 2   & 4.9 &  7.8   & 1.8 & 11.5   & 1.9 & 7.2   & 0.7 & 3.8 \\  
    \multirow{1}{*}{$\nicefrac{25}{75}$} 
                          & 8   & 2.3 &  5.1   & 0.9 & 10.1   & 0.2 & 5.9   & 0.1 & 3.9 \\   
                          & 64  & 0.5 &  3.4   & 0.0 & 7.5    & 0.1 & 6.5   & 0.1 & 3.4 \\  
                          & RFT & $-$ &  {\bf 2.0}   & $-$ & {\bf 2.1}    & $-$ & {\bf 5.9}   & $-$ & {\bf 3.4} \\
    %                       \cline{2-4}\\[-0.8em]
    %                       & 2   &  0.5   &  3.7 &  1.1   & 5.6  &  1.0   &  1.2 & 0.2 & 1.6  \\   
    % \multirow{1}{*}{1.00} & 8   &  0.4   &  1.3 &  0.5   & 6.6  &  0.2   &  1.6 & 0.5 & 1.1  \\   
    %                       & 64  &  0.1   &  0.2 &  0.7  &  2.9  &  0.3   &  0.9 & 0.5 & 1.1  \\      
    %                       & FFT &  $-$   &  0.6 &  $-$   &  0.9 &  $-$   &  1.3 & $-$ &  0.5 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{8pt}
  \caption{Harmful bias gap (HBG) on the minority group between regular fine-tuned model (RFT) and LoRA models fine-tuned with different ranks, and Accuracy parity (AP) both in percentage. The results are computed for various unbalanced levels $\nicefrac{\text{Majority}}{\text{Minority}}$.}
\label{tab:class_llm}
\end{table}

\begin{wrapfigure}[18]{r}{0.4\textwidth}
\vspace{-12pt}
      \includegraphics[width=\linewidth]{figures/outputimdb_gpt2.png}\\[-2pt]
        % \caption{GPT-2 on IMDb}
        \includegraphics[width=\linewidth]{figures/outputsst2_gpt2.png}
        % \caption{GPT-2 on SST2}
        %\includegraphics[width=.24\textwidth]{figures/outputimdb_opt.png}
        % \caption{OPT-1.3b on IMDb}
        %\includegraphics[width=.24\textwidth]{figures/outputsst2_opt.png}
        % \caption{OPT-1.3b on SST2}
\vspace{-18pt}
\caption{\small{Decision boundary analysis.}}
\label{fig:boundary}
\end{wrapfigure}
\textbf{Impact on decision boundaries.}
To further appreciate the role of the LoRA fine-tuning rank ion decision-making tasks, we present a qualitative analysis illustrating its impact on the distance from the decision boundary in final LLM decisions. This distance serves as a common proxy in fairness analysis, providing insights into how rank adjustments affect model equity and decision-making fairness \citep{DasRF2024ICML}.
Figure \ref{fig:boundary} displays the soft probabilities of decisions for samples classified as ``positive review'' from the \textsl{IMDb} (top) and \textsl{SST2} (bottom) datasets for the \textsl{GPT-2} model. More detailed analyses involving additional models can be found in Appendix \ref{appendix:sequentialdecisions}. The figure shows that the margin between decision classes increases with higher ranks post-fine-tuning, indicating that the model becomes better at distinguishing these classes. 
While outside the scope of this work, these aspects are also connected with model robustness, as highlighted in \cite{DasRF2024ICML}, and could indicate that LoRA fine-tuned models may be more sensitive to input perturbations.

These observations are important: {\em They highlight that LoRA fine-tuned models, especially at low (but typical) ranks, may bring unwanted fairness issues for downstream tasks.}
